Gravitational lensing reveals ionizing ultraviolet photons escaping from a distant galaxy

During the epoch of reionisation, neutral gas in the early Universe was ionized by hard ultraviolet radiation emitted by young stars in the first galaxies. To do so, ionizing ultraviolet photons must escape from the host galaxy. We present Hubble Space Telescope observations of the gravitationally lensed galaxy PSZ1-ARC G311.6602-18.4624, revealing bright, multiply-imaged ionizing photon escape from a compact star-forming region through a narrow channel in an optically thick gas. The gravitational lensing magnification shows how ionizing photons escape this galaxy, contributing to the re-ionization of the Universe. The multiple sight lines to the source probe absorption by intergalactic neutral hydrogen on scales of no more than a few hundred, perhaps even less than ten, parsec.

==> Letter.1 <==
\line@list@version{7}

